Polyhedral Object Recognition by Indexing

In computer vision, the indexing problem is the problem of recognizing a few objects in a large database of objects while avoiding the help of the classical image-feature-to-object-feature matching paradigm. In this paper we address the problem of recognizing 3-D polyhedral objects from 2-D images by indexing. Both the objects to be recognized and the images are represented by weighted graphs. The indexing problem is therefore the problem of determining whether a graph extracted from the image is present or absent in a database of model graphs. We introduce a novel method for performing this graph indexing process which is based both on polynomial characterization of binary and weighted graphs and on hashing. We describe in detail this polynomial characterization and then we show how it can be used in the context of polyhedral object recognition. Next we describe a practical recognition-by-indexing system that includes the organization of the database, the representation of polyhedral objects in terms of 2-D characteristic views, the representation of this views in terms of weighted graphs, and the associated image processing. Finally, some experimental results allow the evaluation of the system performance.

==> summary.tex <==
\paragraph{Summary --}
The problem of object recognition in computer vision is the problem of
matching object features with image features. Nevertheless, since an object
has many features associated with it and since an
image contains features that do
not necessarily belong to that object, the matching process is a complex
one because of the large size of the set of image-feature-to-object-feature
assignments. Therefore, in the past, the rationale has been to use constraints
-- such as the rigidity constraint -- in order to maintain the number of
assignments as reduced as possible: Therefore, any search process, including
exhaustive search, is likely to be fast enough because it has to visit a few
thousands of nodes rather than millions.

If many objects rather than a single one (as it has often been the case)
are present in a database of objects to be recognized, then the matching-based
recognition becomes intractable because the complexity grows substantially
with the number of features. An indexing process is crucial whenever
the recognition process has to select among many possible
objects. {\em Recognition by indexing} is
therefore the process that attempts to rapidly extract from a large list of
objects, those few objects that fit a group of image features while avoiding
to establish image-feature-to-object-feature assignments.

The approach advocated in this paper capitalizes onto the representation of
3-D objects in terms of 2-D characteristic views and of characterizing such a
view with a number of weighted graphs. An identical graph representation is
extracted from the image of an unknown 3-D scene. A polynomial
characterization of graphs allows us to organize the ``model graphs" into hash
tables. Therefore, recognition consists of computing similar polynomial
characterizations  for the ``image graphs" and of indexing in the pre-stored
hash tables. Finally, a voting process ranks a number of candidate
characteristic views as
potential recognized objects.


